Auto-Parallelizing Large Models with Rhino: A Systematic Approach on Production AI Platform

We present Rhino, a system for accelerating tensor programs with automatic parallelization on AI platform for real production environment. It transforms a tensor program written for a single device into an equivalent distributed program that is capable of scaling up to thousands of devices with no user configuration. Rhino firstly works on a semantically independent intermediate representation of tensor programs, which facilitates its generalization to unprecedented applications. Additionally, it implements a task-oriented controller and a distributed runtime for optimal performance. Rhino explores on a complete and systematic parallelization strategy space that comprises all the paradigms commonly employed in deep learning (DL), in addition to strided partitioning and pipeline parallelism on non-linear models. Aiming to efficiently search for a near-optimal parallel execution plan, our analysis of production clusters reveals general heuristics to speed up the strategy search. On top of it, two optimization levels are designed to offer users flexible trade-offs between the search time and strategy quality. Our experiments demonstrate that Rhino can not only re-discover the expert-crafted strategies of classic, research and production DL models, but also identify novel parallelization strategies which surpass existing systems for novel models.

==> sec/deprecated.tex <==
Graph coarsening can be regarded as adding heuristic constraints in the strategy search problem to reduce the search
space. Grouping a set of instructions into an abstract instruction implies that compatible sharding methods are used
and no communication is allowed inside the group.

A graph coarsening heuristic should strive for the following properties:
\begin{itemize}
    \item \textbf{Acyclic}: To ensure that the coarsened computation graph is still a DAG, the groups should not create
    cycles. Formally, if two instructions $I_1$ and $I_2$ are inside the same group and there exists a path from $I_1$
    to $I_2$ in the original computation graph, then all instructions in the path must also be in the group.
    \item \textbf{Balance}: Only a small number of instructions are computation-intensive, and the exact sharding
    strategy of other instructions have little impacts on the computation time. A graph coarsening heuristic can separate
    the computation-intensive instructions into different groups to preserve the most of the search space. This can be
    done either explicitly (e.g. grouping around operators with top-k computation times\cite{heterog}) or implicitly
    (e.g. try to balance the computation time of groups\cite{alpa}).
    \item \textbf{Small-cut}: As communication may be required for the tensors that connecting different groups,
    minimizing the tensor sizes on the cut usually leads to shorter communication time.
\end{itemize}
